BREEDS: Benchmarks for Subpopulation Shift

We develop a methodology for assessing the robustness of models to subpopulation shift---specifically, their ability to generalize to novel data subpopulations that were not observed during training. Our approach leverages the class structure underlying existing datasets to control the data subpopulations that comprise the training and test distributions. This enables us to synthesize realistic distribution shifts whose sources can be precisely controlled and characterized, within existing large-scale datasets. Applying this methodology to the ImageNet dataset, we create a suite of subpopulation shift benchmarks of varying granularity. We then validate that the corresponding shifts are tractable by obtaining human baselines for them. Finally, we utilize these benchmarks to measure the sensitivity of standard model architectures as well as the effectiveness of off-the-shelf train-time robustness interventions. Code and data available at https://github.com/MadryLab/BREEDS-Benchmarks .

==> impact.tex <==
\section*{Broader Impact}
Robustness to testing conditions is a prerequisite for safe and reliable
deployment of machine learning models in the real-world. 
In this work, we expand the current model evaluation toolkit by providing
benchmarks for assessing robustness to subpopulation shifts.
This allows us to test if models generalize beyond the limited diversity of
their training datasets.

On the positive side, this toolkit serves as a simple testbed that can
pinpoint ways in which our models fail to generalize.
This provides us with an opportunity to improve and debug these models 
before
deployment, hence avoiding catastrophic failures in real-world scenarios.
On the negative side, well-defined benchmarks can provide users with a false
sense of security.
A models that performs well on a range of benchmarks is likely to be trusted 
and deployed in the real-world, despite having blind spots that these
benchmarks do not capture.
It is thus crucial to perceive benchmark progress properly, using it as a
guide, without trusting it blindly.


